Iteratively Prompt Pre-trained Language Models for Chain of Thought

While Pre-trained Language Models (PLMs) internalize a great amount of world knowledge, they have been shown incapable of recalling these knowledge to solve tasks requiring complex & multi-step reasoning. Similar to how humans develop a "chain of thought" for these tasks, how can we equip PLMs with such abilities? In this work, we explore an iterative prompting framework, a new prompting paradigm which progressively elicits relevant knowledge from PLMs for multi-step inference. We identify key limitations of existing prompting methods, namely they are either restricted to queries with a single identifiable relation/predicate, or being agnostic to input contexts, which makes it difficult to capture variabilities across different inference steps. We propose an iterative context-aware prompter, which addresses these limitations by learning to dynamically synthesize prompts conditioned on the current step's contexts. Experiments on three datasets involving multi-step reasoning show the effectiveness of the iterative scheme and the context-aware prompter design.

==> sections/introduction_v0.tex <==
\section{Introduction}

% \boshi{Basic flow: First begin with describing this new paradigm of LM as KBs and in the era of large PLMs. Then move to two critical challenges: restrictions of current successes on simple tasks, and the necessity of using lightweight methods due to the inevitable large PLM scale. However it remains unclear how to bring prompting into the next level. Perhaps look more at chainofthought. \hs{Yeah, refer to chainofthought and be concise in the first two paragraphs. But they have already used System-1 and System-2, so we might avoid these terms in the paper (you could still use them in your presentation).} Similar to KB shemas, we need ways. Query decomposition?}

% \boshi{Then introduce IP and its advantage over traditional static prompting methods. Could be thought of as a generalization of OptiPrompt, where instead of explicitly extracting a relation for each sample, we learn to synthesize appropriate prompts dynamically depending on the current inputs. Each step has different focus. I think perhaps we could directly refer to some attention visualizations here, so people could get some intuition about the motivation early on. I feel those figures are rather intuitive to understand. Finally say a bit about experiments, ablations, etc. and summarize our contributions.}

Recently, there has been increasing evidence showing that large-scale Pretrained Language Models (PLMs) are capable of internalizing a great amount of world knowledge, which leads to investigations on using PLMs as alternatives to traditional knowledge sources (e.g., textual documents, knowledge bases) to solve tasks requiring world knowledge \cite{petroni2019language, roberts2020much, lee2020language}. This new paradigm could yield many advantages over traditional approaches, such as simpler training pipeline design, huge inference speedup and easier model adaptation to different domains. Performance-wise, large PLMs have shown competitive and increasing capabilities on knowledge probing \cite{petroni2019language, shin-etal-2020-autoprompt, zhong2021factual} and other knowledge-intensive tasks such as question answering \cite{roberts2020much} and fact checking \cite{lee2020language} without resorting to any external knowledge source. 

Despite the encouraging results, current successes in this scheme are restricted to tasks which only require \emph{simple} inference procedures to solve. Studies such as \cite{talmor2020olmpics, kassner2020pretrained, rae2021scaling} reveal that even though PLMs can internalize a great amount of knowledge, they face difficulties on \emph{reasoning upon their acquired knowledge}. This severely limits their usage in downstream tasks that require \emph{complex, multi-step decision procedures}. In addition, as the PLMs scale up (which is inevitable for larger knowledge storage), lightweight methods for knowledge elicitation are needed, such as prompting \cite{liu2021pre} which shows increasing potential recently. 

% \boshi{there actually are some discussion in previous work about fine-tuning disrupts the implicit knowledge storage, perhaps find more evidence on this and mention it here.} However, it remains unclear how to systematically integrate these methods \hs{`integrate these methods' seems less precise.} in multi-step reasoning tasks without requiring heavy human intervention and heuristics \cite{paranjape-etal-2021-prompting, mishra2021reframing, jiang2020can}.

\begin{figure}[t]
  \centering
    \includegraphics[width=0.48\textwidth]{figures/ProbSetup.png}
  \caption{Prompting PLMs for Multi-step Reasoning. Different from previous work which mainly focus on simple queries where a single piece of knowledge is sufficient, here we aim at complex queries which require extracting multiple pieces of knowledge from the PLM to solve.}
\label{fig:pipeline}
\end{figure}

\hs{we may use a separate paragraph to discuss the notable aspects of our method and advantages over existing ones.} In this paper, we propose Iterative Prompting (IterPrompt), a novel framework for systematically eliciting knowledge from PLMs for tasks involving multi-step inference. Firstly, inspired by previous work \cite{qi-etal-2019-answering, xiong2021answering, pmlr-v139-ren21a}, we propose an iterative procedure which progressively extracts knowledge from PLMs conditioned on previously-gathered knowledge; then we design a novel prompting mechanism which addresses key limitations of previous prompting methods when applied in this iterative scheme. 

To illustrate in more details, consider an example involved with \textit{composition}, an important type of multi-step reasoning, given in Figure \ref{fig:pipeline}. Here, an ideal inference pipeline should go into two consecutive steps: 1) find the ``father'' of the topic entity ``Gwilym Lloyd George'' (\textbf{E1}); 2) locate the birthplace of the entity returned in the first step (\textbf{E2}). From this example, several challenges in applying prompting could be identified. \textit{First}, during different inference steps, suitable filtering must be done for the prompts to focus on different components of the complex query. \textit{Second}, the prompts should appropriately integrate knowledge gathered in previous steps into the current step; for instance, during the second step in this example, the prompts need to combine the entity ``David Lloyd George'' in the returned first step evidence with the unresolved part ``What is the place of birth of ...'' in the query. However, existing prompting techniques are either restricted to queries with a single, identifiable relation/predicate \cite{jiang2020can, petroni2019language, zhong2021factual, shin-etal-2020-autoprompt}, or being agnostic and insensitive to step-wise inputs \cite{lester-etal-2021-power, li-liang-2021-prefix, brown2020language}, both not ideal for our aim.

Our proposed IterPrompt aims to address these limitations. We augment the PLM with a \emph{Prompter}, a model which learns to dynamically synthesize prompts which inquire the PLM for knowledge relevant to the query at hand. At each step, the Prompter learns to process the query and all previously gathered evidence, and composes an appropriate continuous prompt which steers the PLM to return the next piece of knowledge. Like other prompting methods, all parameters of the PLM are kept fixed throughout the learning process; also, as the size of the PLM enlarges, the number of tuned parameters in our method scales comparably with or slower than previous prompting methods.

We conduct experiments on three datasets involving multi-step reasoning, \boshi{perhaps also mention why these three; namely they have the annotations we need} including two recent multi-hop Question Answering datasets: 2WikiMultiHopQA \cite{ho2020constructing} \& R4C \cite{inoue-etal-2020-r4c}, and a scientific dataset on reasoning over taxonomic relations, introduced in \cite{talmor2020leap}. We show that our proposed IterPrompt outperforms baseline methods by notable margins, and conduct both qualitative and quantitative analysis on the faithfulness of the learned prompt behaviors.

==> sections/introduction_v1.tex <==
\section{Introduction}

Recently, there has been increasing work showing that large-scale pre-trained language models (PLMs) are capable of internalizing a great amount of world knowledge, yielding competitive performance on knowledge probing \cite{petroni2019language, shin-etal-2020-autoprompt, zhong2021factual} and other knowledge-intensive tasks such as question answering \cite{roberts2020much} and fact checking \cite{lee2020language}, without resorting to any external knowledge source. %This new paradigm could yield many advantages over traditional approaches, such as simpler training pipeline design, huge inference speedup and easier model adaptation to different domains. Performance-wise, large PLMs have shown  


Despite the encouraging results, other work such as \cite{talmor2020olmpics, kassner2020pretrained, rae2021scaling} reveals that PLMs face difficulties in using their stored knowledge to conduct \emph{complex, multi-step} inferences.
%
%In addition, as the PLMs scale up (which is inevitable for larger knowledge storage), lightweight methods for knowledge elicitation are needed, such as prompting \cite{liu2021pre} which shows increasing potential recently. 
%
% \boshi{there actually are some discussion in previous work about fine-tuning disrupts the implicit knowledge storage, perhaps find more evidence on this and mention it here.} However, it remains unclear how to systematically integrate these methods \hs{`integrate these methods' seems less precise.} in multi-step reasoning tasks without requiring heavy human intervention and heuristics \cite{paranjape-etal-2021-prompting, mishra2021reframing, jiang2020can}.
\begin{figure}[t]
  \centering
    \includegraphics[width=0.48\textwidth]{figures/ProbSetup.png}
  \caption{Prompting PLMs for Multi-step Reasoning. Different from previous work which mainly focus on simple queries where a single piece of knowledge is sufficient, here we aim at complex queries which require extracting multiple pieces of knowledge from the PLM to solve.}
\label{fig:pipeline}
\end{figure}
To illustrate this issue in more detail, consider a question involving \textit{composition}, an important type of multi-step inference, in Figure \ref{fig:pipeline}. The correct inference procedure here involves two connected steps: 1) recall the ``father'' of the topic entity ``Gwilym Lloyd George'' (\textbf{E1}); 2) recall the birthplace of the entity returned in the first step (\textbf{E2}). Previous work \cite{petroni2019language, shin-etal-2020-autoprompt, zhong2021factual, roberts2020much, lee2020language} shows that PLMs can internalize a great amount of single-relation factual knowledge such as \textbf{E1} and \textbf{E2}, but other work \cite{talmor2020olmpics, kassner2020pretrained, rae2021scaling} finds that they fail to use such knowledge to answer more complex questions like Q here. 

In this paper, we study how to shepherd a PLM to recall a series of knowledge that is necessary for multi-step inference, which is similar to how humans develop a train of thought for complex decision making. We propose an iterative prompting framework, named IterPrompt, 
%a novel framework for systematically eliciting knowledge from PLMs for tasks involving multi-step inference. Firstly, inspired by previous work \cite{qi-etal-2019-answering, xiong2021answering, pmlr-v139-ren21a}, we propose an iterative procedure
which progressively elicits knowledge from PLMs conditioned on previously-gathered knowledge. 

There are two challenges in developing this iterative prompting framework: (1) During different inference steps, suitable filtering \hs{I think `filtering' isn't an appropriate word.} must be done for the prompts to focus on different components of the complex query. (2) The prompts should appropriately integrate knowledge gathered in previous steps into the current step; for instance, during the second step in the previous example, the prompts need to combine the entity ``David Lloyd George'' in the returned first step knowledge with the unresolved part ``What is the place of birth of ...'' in the query. 

One might wonder if we can directly apply existing prompting methods \cite{XX}, which have shown impressive performance in probing simple factual knowledge in PLMs, in an iterative fashion. \hs{Such methods usually... Some description about how they work.} As a result, they are either restricted to queries with a single, identifiable relation/predicate \cite{jiang2020can, petroni2019language, zhong2021factual, shin-etal-2020-autoprompt}, or being agnostic and insensitive to step-wise inputs \cite{lester-etal-2021-power, li-liang-2021-prefix, brown2020language}, and cannot address the above challenges. 


%Our proposed IterPrompt aims to address these limitations. 

Therefore, we design a novel prompting mechanism: We augment the PLM with a \emph{Prompter}, a model which learns to dynamically synthesize prompts which inquire the PLM for knowledge relevant to the query at hand. At each step, the Prompter learns to process the query and all previously gathered evidence, and composes an appropriate continuous prompt which steers the PLM to return the next piece of knowledge. Like other prompting methods, all parameters of the PLM are kept fixed throughout the learning process. In addition, as the size of the PLM increases, the number of trainable parameters in our method scales comparably with or slower than previous prompting methods.

We conduct experiments on three datasets involving multi-step reasoning, \boshi{perhaps also mention why these three; namely they have the annotations we need} including two recent multi-hop Question Answering datasets: 2WikiMultiHopQA \cite{ho2020constructing} \& R4C \cite{inoue-etal-2020-r4c}, and a scientific dataset on reasoning over taxonomic relations, introduced in \cite{talmor2020leap}. We show that our proposed IterPrompt outperforms baseline methods by notable margins, and conduct both qualitative and quantitative analysis on the faithfulness of the learned prompt behaviors.

==> sections/introduction_v2.tex <==
\section{Introduction}

Humans can develop a train of thought for complex decision making. For example, when asked the question shown in Figure \ref{fig:pipeline}, which involves \textit{composition}, an important type of multi-step inference, humans apply two steps to derive the final answer: 1) recall the ``father'' of the topic entity ``Gwilym Lloyd George'' (\textbf{E1}); 2) recall the birthplace of the entity returned in the first step (\textbf{E2}). %Can pre-trained language models (PLMs) generate such a train of thought, instead of 

Recently, large-scale pre-trained language models (PLMs) have been shown capable of internalizing a great amount of single-relation factual knowledge such as \textbf{E1} and \textbf{E2}, yielding competitive performance on knowledge probing \cite{petroni2019language, shin-etal-2020-autoprompt, zhong2021factual} and other knowledge-intensive tasks such as question answering \cite{roberts2020much} and fact checking \cite{lee2020language}, without resorting to any external knowledge source. However, other work such as \cite{talmor2020olmpics, kassner2020pretrained, rae2021scaling} reveals that PLMs face difficulties in recalling their stored knowledge for \emph{complex, multi-step} inferences. For example, they struggle with answering complex questions like \textbf{Q}, even if they have memorized \textbf{E1} and \textbf{E2}. 
%
%In addition, as the PLMs scale up (which is inevitable for larger knowledge storage), lightweight methods for knowledge elicitation are needed, such as prompting \cite{liu2021pre} which shows increasing potential recently. 
%
% \boshi{there actually are some discussion in previous work about fine-tuning disrupts the implicit knowledge storage, perhaps find more evidence on this and mention it here.} However, it remains unclear how to systematically integrate these methods \hs{`integrate these methods' seems less precise.} in multi-step reasoning tasks without requiring heavy human intervention and heuristics \cite{paranjape-etal-2021-prompting, mishra2021reframing, jiang2020can}.
\begin{figure}[t]
  \centering
    \includegraphics[width=0.48\textwidth]{figures/ProbSetup.png}
  \caption{Iteratively Prompt a PLM to derive a ``train of thoughts'' for multi-step reasoning. \xiang{We may want to highlight our prompter design, and the PLMs is the same for both cases.}}
\label{fig:pipeline}
\end{figure}
%To illustrate this issue in more detail, consider a question involving \textit{composition}, an important type of multi-step inference, in Figure \ref{fig:pipeline}. The correct inference procedure here involves two connected steps: 1) recall the ``father'' of the topic entity ``Gwilym Lloyd George'' (\textbf{E1}); 2) recall the birthplace of the entity returned in the first step (\textbf{E2}). Previous work \cite{petroni2019language, shin-etal-2020-autoprompt, zhong2021factual, roberts2020much, lee2020language} shows that PLMs can internalize a great amount of single-relation factual knowledge such as \textbf{E1} and \textbf{E2}, but other work \cite{talmor2020olmpics, kassner2020pretrained, rae2021scaling} finds that they fail to use such knowledge to answer more complex questions like Q here. 

Analogous to humans' train of thought for complex decision making, how can a PLM recall a series of knowledge that is necessary for multi-step inference? A direct way would be to fine-tune the PLM, but soon one realizes the practical issue in this approach: PLMs which internalize great amount of knowledge are inevitably large in scale, and fine-tuning all parameters of them would become very costly as they keep scaling up. There's also the potential concern that fine-tuning the PLMs may interfere with their implicit knowledge storage, a phenomenon observed in \cite{wang-etal-2021-generative}. Therefore, lightweight methods for knowledge elicitation which keep the PLM's parameters intact would suit better for our purpose, such as prompting \cite{liu2021pre} which shows increasing potential recently. 

In this paper, we explore an iterative prompting framework, named IterPrompt, 
%a novel framework for systematically eliciting knowledge from PLMs for tasks involving multi-step inference. Firstly, inspired by previous work \cite{qi-etal-2019-answering, xiong2021answering, pmlr-v139-ren21a}, we propose an iterative procedure
which progressively elicits knowledge from PLMs for multi-step reasoning tasks.

There are two challenges in developing this iterative prompting framework: (1) During different inference steps, suitable filtering \hs{I think `filtering' isn't an appropriate word.} must be done for the prompts to focus on different components of the complex query. (2) The prompts should appropriately integrate knowledge gathered in previous steps into the current step; for instance, during the second step in the previous example, the prompts need to combine the entity ``David Lloyd George'' (knowledge recalled in the first step) with the unresolved part ``What is the place of birth of ...'' in the query. %in the returned first step knowledge 

One might wonder if we can apply existing prompting methods \cite{petroni2019language, shin-etal-2020-autoprompt, jiang2020can, zhong2021factual, li-liang-2021-prefix, lester-etal-2021-power}, which have shown impressive performance in probing simple factual knowledge in PLMs, in an iterative fashion. \hs{Such methods usually... Some description about how they work.} As a result, they are either restricted to queries with a single, identifiable relation/predicate \cite{jiang2020can, petroni2019language, zhong2021factual, shin-etal-2020-autoprompt}, or being agnostic and insensitive to step-wise inputs \cite{lester-etal-2021-power, li-liang-2021-prefix, brown2020language}, and cannot address the above challenges. 

%Our proposed IterPrompt aims to address these limitations. 

Therefore, we design a novel prompting mechanism: We augment the PLM with a \emph{Prompter}, a model which learns to dynamically synthesize prompts which inquire the PLM for knowledge relevant to the query at hand. At each step, the Prompter learns to process the query and all previously gathered evidence, and composes an appropriate continuous prompt which steers the PLM to return the next piece of knowledge. Like other prompting methods, all parameters of the PLM are kept fixed throughout the learning process. In addition, as the size of the PLM increases, the number of trainable parameters in our method scales comparably with or slower than previous prompting methods.

We conduct experiments on three datasets involving multi-step reasoning, \boshi{perhaps also mention why these three; namely they have the annotations we need} including two recent multi-hop Question Answering datasets: 2WikiMultiHopQA \cite{ho2020constructing} \& R4C \cite{inoue-etal-2020-r4c}, and a scientific dataset on reasoning over taxonomic relations, introduced in \cite{talmor2020leap}. We show that our proposed IterPrompt outperforms baseline methods by notable margins, and conduct both qualitative and quantitative analysis on the faithfulness of the learned prompt behaviors.

==> sections/introduction_v3.tex <==
\section{Introduction}
\label{sec:intro}

Humans can develop a ``train of thought'' for complex decision making. For example, when asked the question shown in Figure \ref{fig:pipeline}, which involves \textit{composition}, an important type of multi-step inference, humans apply two consecutive steps to derive the final answer: 1) find the ``father'' of the topic entity ``Gwilym Lloyd George'' (\textbf{E1}); 2) find the ``birthplace'' of the entity returned in the first step (\textbf{E2}). %Can pre-trained language models (PLMs) generate such a train of thought, instead of 

Recently, large-scale pre-trained language models (PLMs) have been shown capable of internalizing a great amount of factual knowledge such as \textbf{E1} and \textbf{E2}, yielding competitive performance on a range of knowledge-intensive tasks without resorting to any external knowledge source \cite{petroni2019language, shin-etal-2020-autoprompt, zhong2021factual, roberts2020much, lee2020language}. However, work such as \cite{talmor2020olmpics, kassner2020pretrained, rae2021scaling} reveals that PLMs face difficulties in \textit{recalling} relevant knowledge for \emph{complex, multi-step} inferences. For example, they struggle with answering complex questions like \textbf{Q}, even though they have memorized \textbf{E1} and \textbf{E2}. \hs{there seems to be a gap here: (1) how are the methods compared with the methods mentioned below? Do they use the same kind of methodology? (2) we already say `face difficulties in XX', but still throw out a question in the paragraph below.}
%
%In addition, as the PLMs scale up (which is inevitable for larger knowledge storage), lightweight methods for knowledge elicitation are needed, such as prompting \cite{liu2021pre} which shows increasing potential recently. 
%
% \boshi{there actually are some discussion in previous work about fine-tuning disrupts the implicit knowledge storage, perhaps find more evidence on this and mention it here.} However, it remains unclear how to systematically integrate these methods \hs{`integrate these methods' seems less precise.} in multi-step reasoning tasks without requiring heavy human intervention and heuristics \cite{paranjape-etal-2021-prompting, mishra2021reframing, jiang2020can}.
\begin{figure}[t]
  \centering
    \includegraphics[width=0.48\textwidth]{figures/Intro_v1.png}
  \caption{Our Iterative Prompting Approach for deriving a ``train of thoughts'' with PLM (on the right), compared with standard knowledge probing (on the left).}
\label{fig:pipeline}
\end{figure}
%To illustrate this issue in more detail, consider a question involving \textit{composition}, an important type of multi-step inference, in Figure \ref{fig:pipeline}. The correct inference procedure here involves two connected steps: 1) recall the ``father'' of the topic entity ``Gwilym Lloyd George'' (\textbf{E1}); 2) recall the birthplace of the entity returned in the first step (\textbf{E2}). Previous work \cite{petroni2019language, shin-etal-2020-autoprompt, zhong2021factual, roberts2020much, lee2020language} shows that PLMs can internalize a great amount of single-relation factual knowledge such as \textbf{E1} and \textbf{E2}, but other work \cite{talmor2020olmpics, kassner2020pretrained, rae2021scaling} finds that they fail to use such knowledge to answer more complex questions like Q here. 

Analogous to humans' train of thought for complex decision making, how can a PLM recall a series of knowledge that is necessary for multi-step inference? A direct way would be to fine-tune the PLM, but soon one realizes the practical issue in this approach: PLMs which internalize great amount of knowledge are inevitably large in scale, and fine-tuning all parameters of them would become very costly as they keep scaling up. There's also the potential concern that fine-tuning PLMs may interfere with their implicit knowledge storage, a phenomenon observed in \cite{wang-etal-2021-generative} which is more generally related to the \textit{catastrophic forgetting} problem of deep learning models \cite{mccloskey1989catastrophic, kirkpatrick2017overcoming}. Therefore, lightweight methods for knowledge elicitation which keep the PLM's parameters intact would be more preferable for our purpose, such as prompting \cite{liu2021pre} which shows increasing potential recently. \hs{Before we introduce `iterative' framework, should we summarize these existing work as `one-turn' framework to contrast with what we're gonna propose?} 

In this paper, we explore an iterative prompting framework (IterPrompt), 
%a novel framework for systematically eliciting knowledge from PLMs for tasks involving multi-step inference. Firstly, inspired by previous work \cite{qi-etal-2019-answering, xiong2021answering, pmlr-v139-ren21a}, we propose an iterative procedure
which progressively elicits knowledge from PLMs for multi-step reasoning tasks. 

There are two major challenges involved in this framework: (1) During different inference steps, the prompts need to focus on different components of the complex query. (2) The prompts should appropriately integrate knowledge gathered in previous steps into the current step; for instance, during the second step in the example in Figure \ref{fig:pipeline}, the prompts need to combine the entity ``David Lloyd George'' (from knowledge recalled in the first step) with the unresolved part ``What is the place of birth of ...'' in the query. 

One might wonder if we can directly apply existing prompting methods in an iterative fashion. However, these methods are either restricted to queries with a single, identifiable relation/predicate \cite{jiang2020can, petroni2019language, zhong2021factual, shin-etal-2020-autoprompt, qin-eisner-2021-learning}, or being agnostic and insensitive to step-wise inputs \cite{lester-etal-2021-power, li-liang-2021-prefix, brown2020language}, and hence not ideal under the above challenges.

We design a novel prompting mechanism towards mitigating these limitations. We augment the PLM with a \emph{Prompter}, a model which learns to \textit{dynamically synthesize prompts} based on the current step context. At each step, the Prompter learns to process the query and all previously gathered evidence, and composes an appropriate prompt which steers the PLM to recall the next piece of knowledge. Like other prompting methods, all parameters of the PLM are kept fixed throughout the learning process. In addition, as the size of the PLM increases, the number of trainable parameters in our method scales comparably with or slower than previous prompting methods.

We conduct experiments on three datasets involving multi-step reasoning, including two recent multi-hop Question Answering datasets: 2WikiMultiHopQA \cite{ho2020constructing} \& R4C \cite{inoue-etal-2020-r4c}, and a scientific dataset on reasoning over taxonomic relations, introduced in \cite{talmor2020leap}. We show 1) the effectiveness of this iterative scheme; 2) our proposed IterPrompt outperforms previous methods by notable margins; and 3) both quantitative and qualitative analysis on the faithfulness of the learned prompt behaviors.

==> sections/methodology_v0.tex <==
\section{Methodology}
Given a complex query $q$, our goal is to drive a PLM $\mathcal{M}$ to recall a sequence of simple knowledge statements $C_q=[c_1,...,c_{n_q}]$ which is sufficient for deciding the response to $q$. In particular, we focus on developing prompting methods, where the parameters of $\mathcal{M}$ are fixed and we aim to construct \xiangadd{prompt $T$}{prompts $T=[t_1,...,t_{n_q}]$} which steer $\mathcal{M}$ to recall $C_q$. Writing \xiangadd{$\mathcal{M}^T$}{$\mathcal{M}^t_i$} as $\mathcal{M}$ augmented with prompt \xiangadd{T}{$t_i$}, our training objective is to learn how to find $T$ which could maximize the log likelihood 

$$
    \mathcal{L}(T)=\sum_{i=1}^N \log P(C_{q_i}|\xiangadd{q_i}{q}; \mathcal{M}^t_i)
$$ 

with a set of training data $\{q_i, C_{q_i}\}_{i=1}^N$. Note that the settings in previous work such as \cite{zhong2021factual, shin-etal-2020-autoprompt, lester-etal-2021-power, li-liang-2021-prefix, qin-eisner-2021-learning} correspond to the reduced case where $|C_q|=1$ for any query $q$. 

\subsection{Iterative Prompting Framework}
Inspired by the sequential nature of multi-step decision tasks, we approach the problem in an iterative way:
$$
    P(C_q|q; \mathcal{M}^T) = \prod_{j=1}^{n_q} P(c_j|q,c_{j-1},...,c_1; \mathcal{M}^T)
$$
where at step $j$, $\mathcal{M}^T$ recalls the next piece of knowledge $c_j$ conditioned on the query $q$ and all previously gathered knowledge $c_{j-1},...,c_1$.

\subsection{Context-Aware Prompter}
%\textbf{Modelling the prompt $T$.} 
Previous prompting methods which take single-relation inputs clearly fail to apply in this iterative setting due to the complexity of the input context $q,c_{j-1},...,c_1$. Task-level prompting methods such as Prompt-Tuning \cite{lester-etal-2021-power} and Prefix-Tuning \cite{li-liang-2021-prefix} are applicable here, where $T$ is treated as a \textit{static} parameter. However, as described earlier, this modelling makes it difficult for $T$ to handle variabilities across different steps. In this work, we model $T$ as the output of \textit{Prompter}, a learnable function mapping $f_\Theta$ which dynamically synthesizes $T$ \textit{w.r.t.} the current step input context:
$$
    T = f_\Theta(q,c_{j-1},...,c_1), \forall j
$$

\noindent \textbf{Prompter Instantiation.} While there are many plausible design choices for the Prompter, here we instantiate it with a transformer language model (detailed illustration in Figure \ref{fig:prompter}). The prompts are designed to be contextualizations (by the Prompter) of a set of special tokens with respect to the current-step input, linearly projected into the PLM's embedding space by a trainable matrix (omitted in the figure due to space considerations). In this work, we adopt Encoder-Decoder PLMs and use prefix-prompts in the implementations, and hence we have prompts that are prepended to both the PLM's encoder inputs and decoder inputs. Note that our design could be easily adapted to other types of PLMs (e.g., encoder-only/decoder-only models) and prompt positionings (e.g., infix).

\begin{figure}[h]
  \centering
    \includegraphics[width=0.48\textwidth]{figures/Prompter.png}
  \caption{Our context-aware prompter design. The prompter contextualizes a set of special tokens \textit{w.r.t.} the current step context $q, c_{j-1},...,c_1$ to get the resulting prompts, which steers the PLM to recall the next piece of knowledge $c_j$.}
\label{fig:prompter}
\end{figure}


\noindent \textbf{Comparison with Prompt/Prefix-Tuning.} As mentioned earlier, both Prompt-Tuning \cite{lester-etal-2021-power} and Prefix-Tuning \cite{li-liang-2021-prefix} model the prompt $T$ as a context-agnostic parameter. In Prompt-Tuning, $T$ has the same identity as in our approach which is a set of virtual input tokens (\textit{Encoder Prompts} \& \textit{Decoder Prompts} in Figure \ref{fig:prompter}). In Prefix-Tuning, $T$ is modelled to be the set of activations (keys \& values in the transformer attention blocks) of the virtual tokens across all PLM layers. Let $D$ be the embedding dimension of the PLM, $h$ be the number of layers in the PLM, $d$ be the embedding dimension of the Prompter and $l$ be the total number of prompt tokens (both encoder \& decoder prompts). As the PLM scales, the number of trainable parameters is $\Theta(d\cdot (D+l))$ for our proposed method, $\Theta(l\cdot D)$ for Prompt-Tuning and $\Theta(l\cdot h\cdot D)$ for Prefix-Tuning. It can thus be seen that our method scales comparatively with Prompt-Tuning, slower than than Prefix-Tuning, and overall maintains a manageable amount of trained parameters as the PLM scales up.

\noindent \textbf{Continuous v.s. Discrete Prompts}. While modelling $T$ as discrete tokens in the PLM's vocabulary could increase the readability of the prompts, a discrete space is much less expressive than its continuous counterpart, and optimization over a discrete space could be highly inefficient. Also, despite being inside the vocabulary, the searched discrete prompts could still have low interpretability as could be seen by the given examples in \cite{shin-etal-2020-autoprompt}. Hence, we follow prior work \cite{zhong2021factual, li-liang-2021-prefix, lester-etal-2021-power, qin-eisner-2021-learning} and model the prompts to be continuous virtual tokens instead of discrete tokens.

% \hs{I am a bit concerned that readers might not be familiar with either approach. It seems these two methods are playing an important role; should we consider adding a background section before `Methodology' to describe clearly what they did? (if we do, we don't need to describe them again in the Exp section.)}

\subsection{Learning and Inference} 

We use teacher-forcing for model training, namely at each step, the ground truth contexts at that step (query and previous knowledge pieces) are presented to the model, and we maximize $\mathcal{L}(T)$ using standard sequence-to-sequence learning objectives. During inference, we proceed autoregressively by feeding the recalled knowledge at step $t-1$ as the additional context at step $t$, and execute for some predefined number of steps.

==> sections/related_v0.tex <==
\section{Related Work}
% \boshi{I think it's better to move this part to the second-last section.}
\subsection{Prompting}
Prompting \cite{liu2021pre} is a new NLP paradigm which has been receiving growing research interests recently. Instead of fine-tuning the PLM on different tasks, prompting methods seek to ``reframe'' tasks into prompts which accord with the PLM's input format, and extract useful information from the predicted results which can be further utilized downstream.

\textbf{Relation-specific prompting.} This line of work mostly follows \cite{petroni2019language} which introduced LAMA, a benchmark for cloze-style factual probing, where each sample is accompanied with one relation. For each relation in the dataset, a separate prompt template is either manually-crafted \cite{petroni2019language}, mined \cite{jiang2020can}, or searched using end supervision \cite{shin-etal-2020-autoprompt, zhong2021factual}. Generally speaking, these methods can only work with simple queries with one single, identifiable relation/predicate.

\textbf{Static prompting.} Another line of work utilize prompting as an alternative way of ``adapting'' PLMs; here the prompts could be thought of as task-level instructions which are static and not sensitive to sample-wise inputs. In prior work, people have explored manually specifying the prompts \cite{brown2020language} and also automatically searching appropriate prompts with gradient-based optimization using end supervision \cite{li-liang-2021-prefix, lester-etal-2021-power}.

\boshi{TODO: perhaps mention some other work which use prompting to (help) solve downstream task. Most of these are manually-created prompts specialized to certain tasks.}

\subsection{Reasoning capabilities of PLMs}
There has been a recent line of work investigating the reasoning capabilities of PLMs \cite{talmor2020olmpics, rogers2020primer, kassner2020pretrained}.

\subsection{Iterative Knowledge Retrieval}
We are inspired by methods that iteratively retrieve knowledge over an explicit knowledge source for multi-step reasoning, mostly in the area of Open-Domain Question Answering \cite{xiong2021answering, qi-etal-2019-answering}. Our problem setting could be thought of as iterative retrieval over implicit knowledge in PLMs instead of over explicit knowledge source.



==> sections/related_v1.tex <==
\section{Related Work}
% \boshi{I think it's better to move this part to the second-last section.}
\noindent\textbf{Eliciting Knowledge from PLMs.}
With the recent success of large-scale pre-trained language models (PLMs), there has been growing interest in investigating what is captured by these PLMs during pre-training~\cite{talmor2020olmpics, rogers2020primer, kassner2020pretrained}. Studies have shown that in addition to learning linguistic knowledge about language use, PLMs are capable of memorizing a great amount of world knowledge~\cite{rogers2020primer}, yielding competitive performance on knowledge probing \cite{petroni2019language, shin-etal-2020-autoprompt, zhong2021factual} and other knowledge-intensive tasks such as question answering \cite{roberts2020much} and fact checking \cite{lee2020language}, without resorting to any external knowledge source. On the other hand, other work such as \cite{talmor2020olmpics, kassner2020pretrained, rae2021scaling} reveals that PLMs still face difficulties in recalling their stored knowledge for \emph{complex, multi-step} inferences, such as answering complex composition questions that. 


We are also inspired by methods that iteratively retrieve knowledge over an explicit knowledge source for multi-step reasoning~\cite{xiong2021answering, qi-etal-2019-answering}. Our problem setting could be thought of as iterative retrieval over implicit knowledge in PLMs instead of over explicit knowledge sources.


\noindent\textbf{Prompt Learning.}
\xiang{Discuss prompt learning methods, including those use discrete or continuous prompts. Mention its application in probing knowledge from PLm and connect to our work.}
Prompting \cite{liu2021pre} is a new NLP paradigm which has been receiving growing research interests recently. Instead of fine-tuning the PLM on different tasks, 
% prompting methods seek to ``reframe'' tasks into prompts which accord with the PLM's input format, and extract useful information from the predicted results which can be further utilized downstream.
prompting as an alternative way of ``adapting'' PLMs; here the prompts could be thought of as task-level instructions which are static and not sensitive to sample-wise inputs. In prior work, people have explored manually specifying the prompts \cite{brown2020language} and also automatically searching appropriate prompts with gradient-based optimization using end supervision \cite{li-liang-2021-prefix, lester-etal-2021-power}. \xiang{A special case is relation-specific prompting ...} This line of work mostly follows \cite{petroni2019language} which introduced LAMA, a benchmark for cloze-style factual probing, where each sample is accompanied with one relation. For each relation in the dataset, a separate prompt template is either manually-crafted \cite{petroni2019language}, mined \cite{jiang2020can}, or searched using end supervision \cite{shin-etal-2020-autoprompt, zhong2021factual}. Generally speaking, these methods can only work with simple queries with one single, identifiable relation/predicate.

\boshi{TODO: perhaps mention some other work which use prompting to (help) solve downstream task. Most of these are manually-created prompts specialized to certain tasks.}

\xiang{Our work differs from prefix-tuning and prompt-tuning, but is similar to context-tuning ...}

\boshi{It occurs to me that our work should be somehow related to intrinsic dimension in fine-tuning.}


==> sections/tables/QA.tex <==
\begin{table}
\centering
\scalebox{0.66}{
    \begin{tabular}{l|}
    \hline
    \\
    \\
    \hline
    \hline
    Oracle-RD \\
      \hline
    PLM-QA \\
      \hdashline
    PLM-FT  \\
    PLM-FT (Iter) \\
      \hline
    Prompt-T \\
    Prompt-T (Iter) \\
      \hdashline
    Prefix-T  \\ 
    Prefix-T (Iter)  \\ 
      \hdashline
    iCAP \\ 
    \hline
    \end{tabular}
    \begin{tabular}{|cc}
    \hline
    \multicolumn{2}{|c}{\textbf{2Wiki}} \\
    EM & F1 \\
    \hline
    \hline
    97.8 & 98.9 \\
      \hline
    $24.1_{\pm 0.2}$ & $29.3_{\pm 0.4}$	\\
      \hdashline
    $33.6_{\pm 0.6}$ & $37.8_{\pm 0.5}$	\\
    $45.5_{\pm 1.4}$ & $50.9_{\pm 1.7}$	\\
      \hline
    $26.9_{\pm 0.6}$ & $31.0_{\pm 0.6}$ \\
    $25.0_{\pm 0.6}$ & $30.2_{\pm 0.2}$ \\ 
      \hdashline
    $31.6_{\pm 0.1}$ & $35.6_{\pm 0.2}$ \\ 
    $31.1_{\pm 0.7}$ & $36.4_{\pm 0.4}$ \\ 
      \hdashline
    $42.8_{\pm 2.5}$ & $47.9_{\pm 2.3}$	\\
    \hline
    \end{tabular}
    \begin{tabular}{c}
    \hline
    \multicolumn{1}{c}{\textbf{LoT}} \\
    EM \\ 
    \hline
    \hline
    100.0 \\ 
      \hline
    $68.3_{\pm 0.4}$ \\ 
      \hdashline
    $76.0_{\pm 0.6}$  \\
    $77.8_{\pm 0.3}$ \\ 
      \hline
    $65.9_{\pm 1.1}$ \\ 
    $68.8_{\pm 1.1}$ \\ 
      \hdashline
    $69.0_{\pm 0.2}$  \\ 
    $72.6_{\pm 0.3}$ \\ 
      \hdashline
    $73.8_{\pm 0.3}$ \\ 
    \hline
    \end{tabular}
    \begin{tabular}{cc|}
    \hline
    \multicolumn{2}{c|}{\textbf{R4C}} \\
    EM & F1 \\ 
    \hline
    \hline
    75.7 & 86.8 \\ 
      \hline
    $22.6_{\pm 0.7}$ & $28.8_{\pm 1.0}$ \\ 
      \hdashline
    $25.3_{\pm 1.2}$ & $36.8_{\pm 0.9}$	\\
    $32.2_{\pm 0.0}$ & $42.5_{\pm 0.5}$ \\ 
      \hline
    $16.6_{\pm 2.9}$ & $25.9_{\pm 2.8}$ \\ 
    $22.4_{\pm 2.3}$ & $30.4_{\pm 2.7}$ \\ 
      \hdashline
    $19.2_{\pm 0.4}$ & $29.2_{\pm 0.5}$ \\ 
    $24.0_{\pm 0.3}$ & $34.2_{\pm 0.4}$ \\ 
      \hdashline
    $25.7_{\pm 1.9}$ & $35.2_{\pm 1.9}$ \\ 
    \hline
    \end{tabular}}
\caption{Results for Extrinsic Evaluation, where the recalled knowledge of each method is used for final inference, except for Oracle-RD and PLM-QA.}
\label{table:qa}
\end{table}

==> sections/tables/recall.tex <==
\begin{table*}[t]
\centering
\scalebox{0.9}{
    \begin{tabular}{l|}
    \hline
    \\
    \\
    \hline
    \hline
    PLM-FT  \\
    PLM-FT (Iter) \\
      \hline
    Prompt-T  \\ 
    Prompt-T (Iter)  \\ 
      \hdashline
    Prefix-T  \\
    Prefix-T (Iter) \\
      \hdashline
    iCAP \\ 
    \hline
    \end{tabular}
    \begin{tabular}{|cccc}
    \hline
    \multicolumn{4}{|c}{\textbf{2Wiki}} \\
    \textbf{Ent.}$R^*$ & \textbf{Ent.}$R$ & \textbf{Ans.}$\hat{R}$ & \textbf{Ans.}$R$ \\
    \hline
    \hline
    $10.3_{\pm 0.6}$ & $33.8_{\pm 1.4}$ & $12.3_{\pm 1.4}$ & $45.3_{\pm 1.6}$\\
    $26.3_{\pm 0.7}$ & $48.9_{\pm 0.6}$ & $35.4_{\pm 0.7}$ & $60.6_{\pm 0.3}$ \\
      \hline
    $5.5_{\pm 0.1}$ & $22.3_{\pm 0.4}$ & $6.6_{\pm 0.1}$ & $41.3_{\pm 0.6}$\\
    $10.8_{\pm 0.4}$ & $27.5_{\pm 0.5}$ & $16.7_{\pm 0.7}$ & $46.2_{\pm 0.8}$ \\ 
      \hdashline
    $6.7_{\pm 0.1}$ & $25.9_{\pm 0.2}$ & $7.6_{\pm 0.1}$ & $44.2_{\pm 0.1}$\\
    $14.8_{\pm 0.4}$ & $33.9_{\pm 0.5}$ & $22.5_{\pm 0.4}$ & $53.2_{\pm 0.3}$	 \\ 
      \hdashline
    $22.0_{\pm 1.7}$ & $42.1_{\pm 2.2}$ & $28.6_{\pm 2.7}$ & $54.6_{\pm 1.6}$	 \\
    \hline
    \end{tabular}
    \begin{tabular}{cc}
    \hline
    \multicolumn{2}{c}{\textbf{LoT}} \\
    \textbf{Cont.}$R^*$ & \textbf{Cont.}$R$ \\ 
    \hline
    \hline
    $41.8_{\pm 1.2}$ & $70.8_{\pm 0.8}$ \\
    $41.3_{\pm 1.6}$ & $70.1_{\pm 1.2}$ \\ 
      \hline
    $35.3_{\pm 1.6}$ & $62.8_{\pm 1.9}$ \\
    $33.3_{\pm 1.5}$ & $63.4_{\pm 1.8}$ \\ 
      \hdashline
    $31.8_{\pm 0.2}$ & $64.0_{\pm 0.1}$ \\
    $31.6_{\pm 0.3}$ & $64.9_{\pm 0.3}$	 \\ 
      \hdashline
    $34.1_{\pm 0.7}$ & $65.0_{\pm 0.2}$	 \\ 
    \hline
    \end{tabular}
    \begin{tabular}{cc|}
    \hline
    \multicolumn{2}{c|}{\textbf{R4C}} \\
    \textbf{Ans.}$\hat{R}$ & \textbf{Ans.}$R$ \\ 
    \hline
    \hline
    $38.1_{\pm 1.2}$ & $43.9_{\pm 1.1}$\\
    $43.1_{\pm 1.2}$ & $48.5_{\pm 1.0}$\\ 
      \hline
    $28.2_{\pm 0.9}$ & $33.4_{\pm 0.4}$\\
    $30.6_{\pm 2.2}$ & $36.0_{\pm 2.4}$\\ 
      \hdashline
    $27.2_{\pm 0.4}$ & $33.9_{\pm 0.3}$\\
    $33.7_{\pm 0.6}$ & $39.8_{\pm 0.6}$	 \\ 
      \hdashline
    $36.8_{\pm 0.7}$ & $41.5_{\pm 0.6}$	 \\ 
    \hline
    \end{tabular}}
\caption{Results for Intrinsic Evaluation, where ``(Iter)'' indicates the iterative setting of a method. All metrics are defined in \S\ref{evalmetric} and overall measure the gold (answer) entity/object coverage of the recalled knowledge from different perspectives.}
\label{table:recall}
\end{table*}
